APNN-TC: Accelerating Arbitrary Precision Neural Networks on Ampere GPU Tensor Cores

Over the years, accelerating neural networks with quantization has been widely studied. Unfortunately, prior efforts with diverse precisions (e.g., 1-bit weights and 2-bit activations) are usually restricted by limited precision support on GPUs (e.g., int1 and int4). To break such restrictions, we introduce the first Arbitrary Precision Neural Network framework (APNN-TC) to fully exploit quantization benefits on Ampere GPU Tensor Cores. Specifically, APNN-TC first incorporates a novel emulation algorithm to support arbitrary short bit-width computation with int1 compute primitives and XOR/AND Boolean operations. Second, APNN-TC integrates arbitrary precision layer designs to efficiently map our emulation algorithm to Tensor Cores with novel batching strategies and specialized memory organization. Third, APNN-TC embodies a novel arbitrary precision NN design to minimize memory access across layers and further improve performance. Extensive evaluations show that APNN-TC can achieve significant speedup over CUTLASS kernels and various NN models, such as ResNet and VGG.

==> 01_intro_backup.tex <==
\section{Introduction}
% \boyuan{2 pages: abstract + intro}

\boyuan{TODO: Revise the challenges and contributions to match with Figure 1.}

Over the recent years, the demands to improve the performance of the deep neural network (DNNs) have never been satisfied. 
%
Prior work approaches the faster and more efficient DNNs from different aspects, such as model pruning~\cite{liu2020autocompress, niu2020towards, ma2020pconv}, kernel factorization~\cite{mobilenet_2017_howard, sandler2018mobilenetv2, xception}, and data quantization~\cite{training-qnn, qcnn}.
%
Among those efforts, quantization based DNN acceleration~\cite{searchlowbit,training-qnn,qcnn} finding its strengths in minimum modification of the original model architecture, lower memory consumption and better runtime performance.
%
However, existing approaches of enforcing quantization in DNN inference usually face several challenges from different aspects.

Lack of flexibility for choosing different bit representations in DNNs to maximize model accuracy performance gains at the algorithm level.
Work from~\cite{searchlowbit,training-qnn,qcnn} generally maintains the uniform quantization scheme, which applies one bit-width (e.g., 1-bit) to all types of data in DNNs (weights and feature maps). 
This leads to the ignorance of the speciality of data in DNNs requiring different bits of representation for maintaining model accuracy performance, thus, suffering from evident accuracy drop compared with the full-precision counterpart.
% The root cause of triggering this dilemma is the lack of .

\begin{figure} [t] \small
    \centering
    \includegraphics[width=0.5\textwidth]{images/Overview.pdf}
    \caption{The overview of APNN framework. \boyuan{performance analysis to analytic model}}
    \label{fig: The overview of APNN framework.}
    % \vspace{-15pt}
\end{figure}


%
Lack of support for low-bit NN computing at the framework level. 
Existing NN computing frameworks usually support limited choice of the quantization bit-width. Take the most famous Pytorch~\cite{pytorch} framework as an example, it can only naturally  their proposed quantization scheme can only work on x86 CPUs with AVX2 support or higher. While deploying the Pytorch on the more powerful GPU devices, it still requires to rely on the full-precision model, thus, wasting most computation power.

Lack of effective low-level computation operator support at the device. 
Existing hardware devices, such as CPU and GPU operates at the level of individual bytes. 
Even lower-bit computation~\cite{rastegariECCV16,bnn,lin2017towards} looks feasible with stunning theoretical performance from the algorithm perspective, implementation them on the CPU/GPU devices requires non-trivial efforts, some efforts achieves this via the bit-level simulation, which is a ``fake'' low-bit that still operating on byte-based data types. Also, insights from previous literature~\cite{li2019bstc,Li2020AcceleratingBN} indicates that low-bit computation, such as binary computation, could hardly utilize the full computation power of GPUs, thus, suffering from even inferior performance.


To this end, we propose, \Mname, the first arbitrary-precision neural network computing framework on GPU Tensor Core. \Mname~takes the user specification of NN (e.g., the layer structure and the weight/feature bit-width) as the input and then customize our optimized kernel template for efficient execution on GPU Tensor Core. 
Unlike previous fixed-bit design that only support limited number of bit-width choices, \Mname~can support arbitrary-bit precision at both layer and component granularity, i.e., different layers could have different bit-width while weights and feature maps can differ in their bit-width. 
In addition, \Mname~is targeted on high-performance GPU devices with the lately introduced Tensor Core Unit with a set of kernel-level optimization such as the novel batching strategy, which can maximize its performance gains. 
More importantly, \Mname~is built on the natively supported 1-bit Tensor Core computation of CUDA, thus, enjoying from both the memory saving and high-performance execution. 
In summery, we make the following contributions in this paper.
\begin{itemize}
    \item We propose and implement a brand-new  arbitrary-bit data representation and computation scheme based on bit-level operation for generic NN computation, such as Linear transformation and Convolution.
    \item We craft a highly efficient GPU kernel design based on a novel multi-dimensional batching strategy to exploit the performance potential of GPU Tensor Core in our arbitrary-bit NN algorithm design.
    \item We further incorporate an effective design space explore scheme to determine the value of configuration variables for a better runtime performance.
    \item Extensive experiments show that \Mname~can consistently maintain runtime performance advantages (averaged $\times$ faster) over the highly-engineered low-bit computation library CUTLASS across mainstream NN models. 
\end{itemize}

==> 03_APKernel_Backup.tex <==
\section{Arbitrary Precision Layer Design}
% \boyuan{1.5 page}

In this section, we propose the Arbitrary-Precision Matrix Multiplication (APMM) for fully connected layers and Arbitrary-Precision Convolution (APConv) for convolution layers.
% We will first focus on the kernel design for APFC and then discuss APConv as an extension.
% Finally, we will include a performance model and auto-tuning to further improve the performance.
% Figure \ref{fig: The overview of APNN framework.} shows an overview of our arbitrary precision kernel design.
% First, we conduct \textit{bit-decoding} to split the arbitrary precision input matrices into 1-bit matrices.
% Then, we will compute with 1-bit matrices and use \textit{bit-encoding} to generate the computation results in 32-bit format. 

% \boyuan{Add a figure and discussion on the overall flow. So we can describe top-to-down.}


% Memory space complexity $\mathcal{O}(input\_bit\times weight\_bit\times T_m \times T_n\times T_k)$
%  \begin{algorithm}[h]
%   \caption{Bit Decomposition. (Bit\_Decompose)}
% \SetAlgoLined
%   \SetKwInOut{Input}{input}
%   \SetKwInOut{Output}{output}
%   \Input{Matrix A with $M$-bit precision}
%   \Output{Matrix list of A for M < 4 or Matrix tuple list (mat, bit\_size, bit\_pos) of A for M $\geq$ 4.}
%   \uIf{M $<$ 4}{ \tcp{single mode.}
%     A\_list = Single\_Bit\_Decompose(A)\;
%   }
%   \uElse{ \tcp{mixed mode.}
%     \tcp{Two modes for mixed-bit decomposition (M > 4).}
%     \tcp{Mode-1: larger-bit first (lb), 10 --> 8 + 2.}
%     A\_tuple\_list = Mixed\_Bit\_Decompose(A, mode='lb')\;
%     \tcp{Mode-2: more-trunk first (mt), 10 --> 4 + 4 + 2.}
%     A\_tuple\_list = Mixed\_Bit\_Decompose(A, mode='mt')\;
%   }
% \end{algorithm}
% \begin{figure*} \small
%    \centering
%    \includegraphics[width=0.7\textwidth]{images/batching_strategy.pdf}
%     \vspace{-10pt}
%     \caption{APNN Batch Strategy.}
%     \label{fig: APNN Batch Strategy}
% \end{figure*}



\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{images/APMMIllustration.pdf}
    \vspace{-10pt}
    \caption{Illustration of APMM. GL: GLobal memory. SHMEM: SHared Memory. FRAG: FRAGment.}
    \vspace{-13pt}
    \label{fig:APMMIllustration}
\end{figure*}



\subsection{Arbitrary-Precision Matrix Multiplication (APMM)} \label{sec:APMM}
% \boyuan{First few sentences: Specify the functionality: 1-bit decomposed input and 32-bit synchronized output.}

% \boyuan{Discuss basic implementations, especially their pros and cons.}

APMM takes the decomposed $1$-bit weight matrix $W_s$, $s\in \{0,...,p-1\}$, the decomposed $1$-bit feature matrix $X_t, t\in \{0,...,q-1\}$, and computes output matrix $Y = \sum_{s=0}^{p-1}\sum_{t=0}^{q-1} Y^{(s,t)}*2^{s+t}$.
% where APMM supports two precisions of 32-bit and arbitrary bit.
By default, APMM generates $32$-bit output to avoid data overflow for large matrices and match the $32$-bit output in Tensor Core compute primitives.
APMM also supports arbitrary-precision output when APMM is used as hidden layer in neural networks (NNs) and the output is consumed by the next APMM-based NN layer.

% APFC takes the decomposed 1-bit matrices with shape $M\times K$ and $N\times K$ and generates a 32-bit output matrix of shape $M\times N$.
Considering that APMM essentially computes an arbitrary precision GEneral Matrix-Matrix multiplication (GEMM) kernel with multiple Binary Matrix-MAtrix multiplication (BMMA) kernels, one naive strategy is to build upon existing BMMA kernels \cite{Li2020AcceleratingBN,li2019bstc}.
In particular, we can use existing BMMA kernels to multiply each pair of $W_s$ and $X_t$ and accumulate $W_sX_t$ to the output matrix $Y$.
However, this approach shows significant inefficiency due to two reasons.
First, this approach ignores the data reuse opportunity since the same weight matrix tile from $W_s$ can be multiplied with different feature matrix tile from $X_{t1}$ and $X_{t2}$.
Second, this approach lacks communication across BMMA kernels, such that reducing $W_sX_t$ into $Y$ leads to significant global memory access.
% This would largely 



% there are two naive strategies based on existing 1-bit GEMM implementations.
% There are two naive strategies for APFC, especially when there are several 1-bit GEMM kernels to be executed.
% The first one is to enable the concurrent kernel execution with the stream interface [Citation].
% The second one is to expand the 1-bit GEMM kernel along the z dimension by computing different GEMMs with a unique z-index.


We show our efficient APMM design in Figure \ref{fig:APMMIllustration}.
It includes a \textit{batch-based double caching} to facilitate the data reuse and a \textit{memory-efficient bit compression} to accelerate the accumulation and optionally generating the arbitrary-precision output.
Here, we illustrate the design with $1$-bit $W$ and $2$-bit $X$ for notation simplicity while arbitrary-precision $W$ and $X$ are supported.


% \boyuan{Two key challenges to solve: 1) How to improve the GPU utility, especially when the matrix is small? This is non-trivial and enabled only on Arbitrary-Precision computation compared to 1-bit computation. It could be something similar to "Tiling and Batching" and modified from our current batching strategies (4.1.1).}


\vspace{3pt}
\noindent \textbf{(a) Batch-based Double Caching.}
% Paragraph 1: How to tile.
Batch-based double caching exploits two GPU memory hierarchies (\textit{i.e.}, shared memory and fragment) to cache matrix tiles and facilitate data reuse in APMM computation, as illustrated in Figure \ref{fig:APMMIllustration}(a).
Considering the limited size of shared memory and fragment, we tile weight matrices $W_s$ and feature matrices $X_t$ such that these tiles can be cached in the GPU memory hierarchies.
Formally, given $W_s$ of shape $M\times K$ and $X_t$ of shape $N\times K$, we first tile $W_s$ along the $M$ dimension into block matrix tiles of shape $b_m \times b_k$.
Similarly, we tile $X_t$ along the $N$ dimension into block matrix tiles of shape $b_n \times b_k$.
Here, each GPU block will multiply one pair of block matrix tiles and generate a output matrix tile $b_m \times b_n$.
Considering that Tensor Cores compute at the warp level, we further tile the $W_s$ into warp matrix tiles of shape $w_m\times w_k$ and the $X_s$ into $w_n \times w_k$ such that each warp computes an output tile of shape $w_m \times w_n$.
To match with the $8\times8\times 128$ \texttt{bmma} compute primitive of Tensor Core, each warp will slide along the $w_m$, $w_n$, and $K$ dimension during computation.
Note that these tiling sizes have significant impact on the performance, which will be analyzed in Section \ref{sec:performanceAnalysis}.


% Paragraph 2: Batch strategy.
Batch-based double caching first adopt a batch strategy to improve inter-thread parallelism and achieve high performance.
Existing work on binary neural networks \cite{li2019bstc,Li2020AcceleratingBN} reports that the GEMM size in NN workload is usually small (\textit{e.g.}, $512\times 512$) such that small matrix tiling sizes (\textit{e.g.}, $32\times 32$) to improve the inter-thread parallelism.
However, this approachs lead to low intra-thread parallelism and prevents data reuse.
Instead, our batch strategy virtually transform multiple small BMMAs into a large BMMA.
In particular, given $W_s, s\in\{1,...,p-1\}$ of shape $M\times K$ and $X_t, t\in \{1,...,q-1\}$ of shape $N\times K$, we batch these small matrices into $W_{B}$ of shape $pM \times K$ and $X_B$ of shape $qN \times K$ and computes with a single large BMMA.
Here, we implement as a ``virtual" batch strategy during the data loading procedure by dynamically deciding the global memory address of the corresponding matrix tile, such that no additional memory movement is involved.

% Paragraph 3: Which data is stored in the shared memory? Why?
Batch-based double caching then exploits two GPU memory hierarchies to facilitate the data reuse at different levels.
The first level is a shared memory caching to reuse matrix tiles from $W_s$ and $X_t$.
% Here, a naive strategy is that each warp independently i) loads a weight tile of shape $w_m\times w_k$ and a feature tile of shape $w_n \times w_k$ for computation, ii) iterates through the K dimension for $K/w_k$ times.
% leading to xxx global memory access.
% \begin{equation*}
% \end{equation*}
Here, a naive strategy is that each warp independently loads a weight tile and a feature tile for computation.
However, we observe that the same weight tile may be multiplied with feature tiles from different 1-bit feature matrices $X^{(0)}$ and $X^{(1)}$, as illustrated in Figure \ref{fig:APMMIllustration}(a).
To this end, our design requires all warps to first collaboratively load $b_m\times b_k$ weight data and $b_n\times b_k$ feature data from global memory to shared memory.
Then, each warp fetch its own matrix tiles from shared memory.
% Instead, we load xxx simultaneously and cache these data matrix in the shared memory to enable data reuse.
In this way, we can significantly reduce the global memory access by exploiting the fast shared memory.

% accelerate the memory access since shared memory is usually xxx faster than global memory.






% Paragraph 4: Which data is stored in Fragment? Why?
The second level is a fragment caching to continuously store the output tiles in the same Tensor Core fragment.
Since Tensor Core compute primitives require to accumulate in 32-bit Tensor Core fragment, the output tiles usually consume large memory space compared with the 1-bit input data.
% In particular, a single warp consumes $w_m\times w_k + w_n\times w_k$ bit to store the weight tile and the feature tile, while using $32 w_m\times w_n$ bits 
Moving the output tiles between shared memory and Tensor Core Fragment may lead to heavy shared memory access.
Moreover, existing dissecting works [Citation] reveal that Fragment is composed of registers and one GPU block of 8 warps can provide upto 256 KB Fragment, which is much larger than shared memory.
To this end, as iterating through the K dimension during computation, we continuously use multiple Fragments to cache the output tiles of shape $b_m \times b_n$ to reduce shared memory access and cache more feature and weight tiles in shared memory.

% continuously cache the same output tile in the same fragment



% cache multiple output tiles in different fragment 










% \boyuan{2) How to efficiently conduct bit-reduction? What is the input (32-bit), the data layout design, and thread utilization? How to avoid unnecessary SHMEM read and write? How to reduce the atomic operations? This is highly related to the Arbitrary-Precision computation and could be modified from our current "Fragment-Enhanced Bit Reduction" (4.1.2).}

\vspace{3pt}
\noindent \textbf{(b) Memory-efficient Bit Compression.}
% Paragraph 1: What is the functionality of memory-efficient bit compression?
% Bit compression takes the 32-bit BMMA outputs and reduces to the APMM outputs, which can be 32-bit or arbitrary-precision.
Bit compression consumes 32-bit BMMA outputs $Y^{(s,t)} \in \text{\texttt{uint32}}^{M\times N}$ and generates $32$-bit APMM outputs $Y\in \text{\texttt{uint32}}^{M\times N}$ as $Y = \sum_{s=0}^{p-1}\sum_{t=0}^{q-1} Y^{s,t}*2^{s+t}$.
Bit compression can also generate arbitrary precision output when it is utilized as NN hidden layers and its output is consumed by the next NN layer.
Overall, bit compression takes only $O(pqMN)$ computation complexity, which is significantly lower than the computation complexity of the GEMM operation.


However, there are two potential memory bottlenecks in bit compression, which have significant impact on the performance.
The first one is the global memory access when reducing $32$-bit BMMA outputs to $32$-bit APMM outputs.
In a naive implementation that independently conducts BMMA and bit compression, bit compression usually introduces similar latency as the BMMA kernel (see Figure \ref{fig:kernelFusionBenfitsEncoding} in evaluation).
The main reason is that, while Tensor Cores provides significantly higher computation throughput than CUDA Cores, the global memory bandwidth remains the same.
The second one is the shared memory access when converting $32$-bit APMM outputs to arbitrary-precision outputs.
In this procedure, we usually need to pack low-bit values (\textit{e.g.}, 2-bit) in registers from different threads to a single memory-aligned value (\textit{e.g.}, 32-bit) before storing to global memory.
Relying on shared memory for data exchange across threads may lead to heavy shared memory access.



% Paragraph 3: Our design includes two parts to mitigate the global memory access and the shared memory access at different computation stages. The first one is xxx. Why it saves global memory access.

Memory-efficient bit compression includes two novel designs to mitigate the memory overhead.
The first design includes a semantic-aware workload allocation and a in-shared-memory reduction.
In particular, at the data loading phase of BMMA, we load feature tiles and weight tiles of the same semantic index such that their multiplication outputs can be reduced directly.
As illustrated in Figure \ref{fig:APMMIllustration}, instead of loading a $b_n \times b_k$ feature tile of $X^{0}$ or $X^{(1)}$, we load two $0.5b_n \times b_k$ feature tiles of both $X^{0}$ and $X^{(1)}$ with the same matrix index.
In this way, we can reduce $WX^{(1)}$ and $WX^{(0)}$ directly in shared memory and mitigate the global memory access while not degrading the BMMA performance.



% is a kernel fusion strategy by bit-encoding in the shared memory before writing to the global memory.
% the bit-encoding with kernel fusion by accumulating the 
% In particular, we first reorganize the data layout such that the BMMA kernel loads elements corresponding to various bits of the same arbitrary-precision element.
% Then, once BMMA kernel stores the intermediate results in the shared memory (\textit{e.g.}, a $64\times 64$ matrix tile), we will conduct the bit-encoding by combining related elements with bit shift and addition.
% For example, for 2-bit weight and 2-bit feature, we will reduce the $64\times 64$ matrix tile to a $32\times 32$ matrix tile in the shared memory.
% Formally, for $p$-bit weight, $q$-bit feature, and matrix tile $b_m \times b_n$, we generate a matrix of shape $b_m\times b_n /(pq)$ to store the encoded results.
% Finally, we store the reduced matrix to the global memory.
% Note that this global memory write is reduced by $pq\times$
% have done xxx. \boyuan{Add one figure illustration and some formulas.}
% Surprisingly, kernel fusion with GEMM and bit-encoding takes lower latency than computing only the GEMM kernels, as shown in Figure \ref{fig:kernelFusionBenfitsEncoding}.
% The reason is that kernel fusion reduces $pq\times$ global memory write by writing only the encoded 32-bit matrix of shape $M\times N$ to the global memory, compared with "GEMM only" that writes $p\times q$ 32-bit matrices of shape $M\times N$.



% Paragraph 4: The second one is xxx. Why it saves shared memory access.
The second design incorporates an element-wise routine and a inter-thread communication to packing low-bit values and mitigate shared memory overhead.
The element-wise routine is an user-defined interface to provide diverse support of quantization and batch normalization across NN layers.
This routine applies on individual 32-bit reduced values in registers.
Given a 32-bit value in a register, this routine may quantize it into a $p$-bit value that is still stored in the 32-bit register with the first $32-p$ bits are zeros.
This routine also includes bit decomposition (Equation \ref{eq:bitDecomposition}) that splits this $p$-bit value in a register to $1$-bit values in $p$ registers.
After that, we use a \texttt{\_\_ballot\_sync} API to enable inter-thread communication and directly pack the $1$-bit values across threads into $32$-bit values that can be stored to global memory.











% \subsubsection{AP-Bit Utilities and Data Organization}


% \boyuan{Besides TC operators, we still need several AP-Bit utilities, such as decomposition and packing. This is non-trivial if we want to reduce the number of atomic operations.}

% \boyuan{We also need data layout design.}



% \boyuan{Yuke: Please fill in this part.}
% \textbf{Bit Decomposition}
% Bit-decomposition here requires a two steps in \Mname. The first step is to quantize the value based on the full-precision input feature map or weight in NN model. 
% As shown in Equation~\ref{}, we can get the quantized model and inputs according to the predetermined bit-width configuration.
% Formally, given a quantization bit $q$ and the 32-bit matrix (weight or feature map matrix) with the shape of $M\times N$, we quantize it as a q-bit data as 
% \begin{equation} \small \label{eq:scale_quantize}%     \alpha^{(q)} = \floor*{\frac{\alpha - \alpha_{min}}{scale}}.
% \end{equation}
% where $\alpha_{min}$ is an empirical lower bound of the matrix values, $scale$ is the ratio between the matrix range and the q-bit representation range, and $\floor*{\cdot}$ is the floor function. 
% \todo{check paper for evaluation}
% The second step is to decompose the individual bits from the quantized matrix through bit shifting as 
% \begin{equation} \small \label{eq:scale_quantize}
%     \alpha^{(q)}_{dec} = \left\{(\alpha^{(q)}_i \gg i) \& 1 \vert \ i < q, i\in \mathbb{Z}^{\dagger} \right\}
% \end{equation}
% where $\alpha^{(q)}_{dec}$ is the set of the 1-bit matrices after bit decomposition. Here, we have $q$ 1-bit matrices with $M\times N$ shape. $(\alpha^{(q)}_i \gg i) \& 1$ will get the $i$-th bit from the 32-bit quantized matrix through bit left-shifting ($\gg$) and bit-wise \texttt{and} operation ($\&$). $\mathbb{Z^{\dagger}}$ is the positive integer domain. 
% \begin{figure} \small
%     \centering
%     \includegraphics[width=0.5\textwidth]{images/matrix_size.pdf}
%     \caption{Matrix sizes in M, N, and K for CNNs. Left: VGG16, Right: ResNet18.\boyuan{Too ugly.}}
%     \label{fig: Matrix sizes in M, N, and K for CNNs.}
% \end{figure}

% \textbf{Data Layout} Data in the \Mname~is organized in a hardware friendly way for benefiting execution performance. Input data of the input layer is 32-bit single-precision floating point, while the data transferring between hidden layers are in low-bit format, for example, we will have $q \times M\times N$ for a $M\times N$ matrix with $q$-bit representation. The quantization and the bit-composition steps are carried out ahead of the input layer or at the end of each hidden layer to reduce the unnecessary data movements among layers. The output layer will not carry the quantization and bit-decomposition, thus, directly generating the 32-bit results for the following classification (such as softmax).



\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{images/channelMajorDataOrganization.pdf}
    \vspace{-10pt}
    \caption{Illustration of Channel Major Data Organization (NPHWC). P indicates the number of bits. $I_{chw}$ indicates the image pixel at the $c$-th channel, $h$-th height, and $w$-th width.}
    \vspace{-10pt}
    \label{fig:channelMajorDataOrganization}
\end{figure}


\subsection{Arbitrary-Precision Convolution (APConv)}
APConv takes the decomposed 1-bit weight matrix $W_s$ of shape $C_{out} \times C_{in} \times K\times K$, the decomposed 1-bit feature matrix $X_t$ of shape $BS \times C_{in} \times Height \times Width$, and generates output matrix $Y$.
Here, $C_{out}$ is the number of output channels, $C_{in}$ is the number of input channels, $K$ is the kernel size, $BS$ is the batch size.

Existing works on bit-level convolution usually adopts a direct convolution design \cite{li2019bstc,Li2020AcceleratingBN} to improve the GPU utilization.
However, these methods ignore the data reuse opportunity and introduces heavy global memory access.
In addition, APConv on a $p$-bit weight and a $q$-bit feature usually has $pq\times$ workload than the BConv on the same weight and feature size, which can easily lead to high GPU utilization.
To this end, APConv incorporates the batch-based double caching design as APMM to mitigate the global memory access.

However, there are still two key challenges that distinguishes APConv from APMM.
The first is the data organization coming where naively reading the $K\times K$ feature map may easily lead to un-coalesced memory access.
The second is the data padding where simply padding zero may lead to errorneous results.
To tackle these challenges, we propose \textit{channel-major data organization} and \textit{input-aware padding design}.

% \boyuan{First few sentences: Specify the functionality: 1-bit decomposed input and 32-bit synchronized output.}

% \boyuan{Discuss basic implementations, especially their pros and cons. Li Ang's SC utilizes direct convolution.}
% \boyuan{We should provide some formula for convolution, just in case the reviewer is not familiar with convolution (highly possible!)}

\vspace{3pt}
\textbf{(a) Channel-Major Data Organization.}
% \boyuan{This is the first difference from the APMM. Need figures to discuss different data organization, pros and cons. The key concept is the coalesced memory access.}
Channel-major data organization transforms un-coalesced and unaligned memory access to a coalesced and aligned one for improving the performance.
Traditional data organization [citation] for $32$-bit convolution usually employs a NCHW design, as illustrated in Figure \ref{fig:channelMajorDataOrganization}(a).
However, naively borrowing this design to APConv leads to un-aligned and un-coalesced memory access due to two reasons.
First, multiple $P$-bit (\textit{e.g.}, 3-bit) elements usually cannot be packed into an aligned 32-bit element, which is required for GPU read and write.
Using a 32-bit element to store a $p$-bit element will introduce extra memory overhead.
Second, convolution operation usually read only $K$ continuous elements (or $KP$ bits) due to the $K\times K$ kernel size, which may lead to un-coalesced memory access. 

We design a channel-major data organization as illustrated in Figure \ref{fig:channelMajorDataOrganization}(b).
There are two key design choices.
First, we split a $P$-bit feature matrix into $P$ 1-bit feature matrices and store each 1-bit feature matrix consecutively.
In this way, we can provide aligned memory access for each 1-bit feature matrix and support arbitrary precision $P$.
Second, we consecutively store all channels of the elements with the same spatial location.
Since convolution layers usually have $128c, c\in \mathcal{N}$ channels, this usually leads to coalesced memory access during computation.





\vspace{3pt}
\textbf{(b) Input-aware Padding Design.}
Input-aware padding design adaptively adjust the padding value according to the input value.
As mentioned in Section \ref{sec:dataAdaptiveOperatorSelection}, when the weight W encodes $-1$ and $1$ with $0$ and $1$, we cannot naively padding $0$ since $0$ represents $-1$.


We propose three padding strategies according to the input data.
First, when both weight and feature encode $0$ and $1$, we simply pad zero for features.
In this case, padding $0$ for features will only add extra $0$ for arbitrary weight values, which does not change the computation result.
Second, when both weight and feature encode $-1$ and $1$, we pad $1$ for features and use an extra \texttt{counter} flag to track the number of $0$s when the convolution weight moves outside the input image frame.
We will minus \texttt{counter} to amend the corresponding convolution result.
Third, when weight encodes $-1$ and $1$ and feature encodes $0$ and $1$, we pad $0$ to features and does not change the convolution results.
















\iffalse
\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c}
    \hline
         &  TLP & Compute Intensity& K Occupancy\\
         \hline \hline
        KM &  & & \\
        KN &  & & \\
        MN && &\\
        \hline
    \end{tabular}
    \caption{Performance Model}
    \label{tab:performanceModel}
\end{table}
\fi




% In this subsection, we want to say two things:
% 1. Tiling size: b_m, b_n, b_k. Significant impact on TLP and ILP.
% 2. Hybrid: int-1-based arbitrary precision, or int4. Peak performance.



\subsection{Performance Analysis} \label{sec:performanceAnalysis}
In our \Mname~kernel design, there are two tuning knobs.
The first one is the block tiling sizes $b_m$, $b_n$, $b_k$.
These block tiling sizes bring trade-off between the thread level parallelism (TLP) and the Instruction level parallelism, especially the compute intensity (CI).
Here, we focus on block tiling sizes.
We empirically observe that utilizing $8$ warps per block and splitting the block workload evenly across warps provides the best performance (\textit{i.e.}, $w_m = b_m/4$, $w_n = b_n/2$, $w_k=b_k$).
The second one is an automated switch between 1-bit based arbitrary-precision computation and built-in 4-bit or 8-bit computation.
In our profiling, we observe that CUTLASS-INT1 is usually only $1.86\times$ faster than CUTLASS-INT4 and $3.83\times$ faster than CUTLASS-INT8 on RTX 3090
\footnote{We inquired experts in NVIDIA and confirmed this performance.}.
Considering that supporting $p$-bit weight and $q$-bit feature introduces $pq\times$ computation overhead (\textit{e.g.}, $4\times$ overhead for 2-bit weight and 2-bit features), we may potentially be slower when the peak int1 performance is achieved on certain bit combinations.
In this subsection, we first analyze the performance impact from each tuning knob.
Then, we propose an autotuning strategy to maximize the performance.
Since APMM and APConv share the same batch-based double caching strategy, we use the same autotuning for these two kernels.

% To this end, our auwe propose a two-step auto-tuning procedure.
% We first select the tiling size to maximize the performance of APMM and APConv.
% Then, we automatically switch between the APMM, APConv, and built-in compute primitives to maximize the final performance.







% integrates an automated switch to adopting built-in compute primitives in such cases.









% In our {\Mname} kernel design, there are two tuning knobs -- the batching strategy (\textit{i.e.}, KM, KN, MN) and the block tiling size (\textit{e.g.}, $8\times 8$, $16\times 16$, $32\times 32$, and $64\times 64$).
% These tuning knobs bring trade-off between the thread level parallelism (TLP) and the Instruction level parallelism (ILP).
% In this section, we first build a performance model to analyze the impact of tuning knobs on TLP and ILP.
% Then, we propose a heuristic algorithm to automatically select the tuning parameters.






\subsubsection{Performance Model.}

TLP refers to the thread level parallelism in terms of the number of threads in use.
Intuitively, larger TLP can improve the GPU utilization and the kernel performance.
% The TLP is determined by both the batching strategy and the matrix tiling size.
Formally, given a p-bit weight matrix of shape $M\times K$, a q-bit feature matrix of shape $K\times N$, the matrix tiling size $b_m\times b_n$, and $T$ threads per matrix tile, we define the TLP as
\begin{equation} \label{eq:TLP} \small
TLP=
\frac{pM \times qN}{b_m \times b_n} \times T %, \quad \quad \quad \text{for MN Batching}
\end{equation}
% Note that while KN and KM batching provides the same TLP, these two batching strategy
% Overall, we see that batching strategy provides higher TLP than KM batching and KN batching.
Intuitively, larger $b_m\times b_n$ may reduce the TLP, which suggests a small $b_m\times b_n$ especially for small matrices.
% For small matrices, a small $b_m\times b_n$ are usually adopted to improve TLP.




Compute intensity (CI) refers to the ratio of computation over the memory access on each thread block.
We aim to improve the CI for two reasons.
First, a higher CI indicates less memory access and better performance.
While the amount of computation remains the same, the amount of memory access may be reduced significantly by data reusing and hyper-parameter tuning.
Second, a higher CI on a thread block provides more opportunities for latency hiding.
Formally, for a matrix tile, we compute the amount of global memory access as $b_m \times b_k + b_n \times b_k$ when reading a $b_m\times b_k$ weight tile and a $b_m\times b_k$ feature tile.
We compute the amount of computation as $2\times b_m \times b_n \times b_k$ from the matrix-matrix multiplication.
Finally, we compute computer intensity as
\begin{equation} \label{eq:CI}\small
    CI = \frac{2\times b_m \times b_n}{b_m + b_n}
\end{equation}
Note that CI can be increased when $b_m$ and $b_n$ are increased.
We also observe that CI is independent of $b_k$ such that we can use smaller $b_k$ to leave space for larger $b_m$ and $b_n$, especially when the shared memory size is a limiting factor.
In our evaluation, we fix $b_k$ as $128$ by default.


The automated switch considers both the peak performance of arbitrary-precision computation and the TLP.
On the peak performance, we profile the ratio of \texttt{int4} peak performance over \texttt{int1} as $R_4$ and the ratio of \texttt{int8} peak performance over \texttt{int1} as $R_8$.
Given a $p$-bit weight and a $q$-bit feature, we define the relative peak performance $R(p,q)=R_4$, if $p\leq4$ and $q\leq 4$; else $=R_8$, if $p\geq 4$ or $q\geq 4$.
Here, $R(p,q)$ is the theoretical upper bound on the peak performance of arbitrary precision computation.
When $pq< R(p,q)$, the peak performance of arbitrary-precision computation is faster than built-in \texttt{int4} or \texttt{int8} since the computation overhead is relatively small.
When $pq > R(p,q)$ but the GPU computation has not been fully exploited (\textit{i.e.}, indicated by a small TLP), we still observe that arbitrary-precision computation achieves better performance than built-in \texttt{int4} or \texttt{int8}.









\subsubsection{Auto-tuning}
We propose a heuristic algorithm for automated selection of block tiling sizes and the automated switch.
% To reduce manual efforts, we transform the autotuning problem on selecting block tiling sizes to an optimization problem and integrate with existing optimization solvers \cite{solver}.
% In particular, we treat the batching strategy (\textit{i.e.}, KM, KN, MN) and the block tiling size (\textit{i.e.}, $b_m, b_n$) as variables.
% To describe the batching strategy in the optimization prblem, we introduce three binary variables $s_1$, $s_2$, and $s_3$ for MN, KN, and KM batching strategies, respectively.
% Then, we require exactly one of $s_i$ to be selected (\textit{i.e.}, set as $1$).
Given the matrix size $M$, $N$, $K$, the weight bit $p$, the feature bit $q$, the algorithm selects $b_m, b_n\in \{16,32,64,128\}$, and the switch in three steps.
First, we compute the TLP of each combination of $b_m$ and $b_n$.
We put these combinations in a priority queue, where a higher TLP leads to a high priority.
Second, we pop individual combinations in the priority queue.
We stick to the first combination with highest TLP if its TLP is already smaller than a threshold $T_{TLP}$.
Otherwise, we continuously pop and select combinations in the priority queue to improve CI while ensuring the TLP is larger than the $T_{TLP}$.
Third, we compare $pq$ with $R(p,q)$.
If $pq<R(p,q)$ or $TLP<T_{TLP}$, we select our APMM and APConv.
We will only select built-in CUTLASS-INT4 and CUTLASS-INT8 when $pq>R(p,q)$ and $TLP>T_{TLP}$.
% Here, we aim to improve the compute intensity (Eq. \ref{eq:CI}) to reduce global memory access and provide more opportunities for latency hiding.
% We also ensure that the TLP (Eq. \ref{eq:TLP}) and the K Occupancy (Eq. \ref{eq:KOcc}) are sufficiently large to fully exploit more thread blocks and allocate more workloads to individual threads.
Here, $R(p,q)$ and $T_{TLP}$ are architecture-specific hyperparameters and only need to be profiled once on each type of GPUs.
On NVIDIA RTX 3090, $R(p,q)$ is $2.5$ for \texttt{int4} and $6$ for \texttt{int8}.
we empirically set $T_{TLP}$ as $??$.



% and $T_2$ to be $???$ abd $???$, respectively.






% Formally, we aim to solve the following optimization problem:
% \begin{equation} \small
%     \begin{split}
%         \max \quad & CI = \frac{2b_m \times b_n}{b_m+b_n} \\
%         s.t. \quad & s_1,s_2,s_3 \in \{0,1\}\\
%         \quad & s_1 + s_2 + s_3 = 1 \\
%         \quad & \frac{pqMN}{b_m b_n}s_1 + \frac{(p+q-1)MN}{b_mb_n}(s_2+s_3) \geq T_1 \\
%         \quad & Ks_1 + pKs_2 + qKs_3 \geq T_2 \\
%     \end{split}
% \end{equation}



% \frac{pM \times qN}{b_m \times b_n} \times T, \quad \quad \quad \text{for MN Batching} \\
% \frac{M \times (p+q-1)N}{b_m \times b_n} \times T, \quad \text{for KN and KM Batching}


% \begin{figure} [t] \small
%     \centering
%     \includegraphics[width=0.5\textwidth]{images/scalar-mm.pdf}
%     \caption{Scalar Arbitrary Precision multiplication Example.}
%     \label{fig: Scalar Arbitrary Precision multiplication Example.}
%     % \vspace{-15pt}
% \end{figure}
% \begin{figure} [t] \small
%     \centering
%     \includegraphics[width=0.5\textwidth]{images/AP_compute_flow.pdf}
%     \caption{The Overall Computation Flow of the APNN GEMM.}
%     \label{fig: The Overall Computation Flow of the APNN GEMM.}
%     % \vspace{-15pt}
% \end{figure}






==> 09_AE.tex <==
% \title{Appendix: Artifact Description/Artifact Evaluation}
% \thispagestyle{empty}
% \maketitle

% \section{Artifact Description \& Evaluation}
\appendix

% \section{Artifact Description/Artifact Evaluation}

\section*{Summary of the experiments reported}
%START_LATEX 
The artifact contains the source code for APNN-TC described in our paper. 
We ran APNN-TC on NVIDIA RTX3090 GPU, and record the execution time of an average of 200 runs. In addition, it contains the shell scripts and instructions needed to carry out other
experiments in the evaluation section of the paper, including
\begin{enumerate}
\item Kernel Evaluation: We evaluate our APNN-TC kernel-level design on different input settings for stand-along GEMM/CONV evaluation and comparison w.r.t the CUTLASS GEMM/CONV kernel implementation.  We report the throughput performance (TFLOPs) for those implementations.
\item Model Evaluation: We evaluate our APNN-TC model-level design on mainstream CNN models, including Alexnet, VGG, and ResNet. And we compare our design w.r.t. CUTLASS-based CNN model in latency (ms) performance.
\item Settings: We run quantized (1-bit, 4-bit, 8-bit, 16-bit, 32-bit) Tensorcore-based GEMM and CONV from CUTLASS-2.4.0 released by NVIDIA on RTX3090 and A100 GPU with CUDA-11.1.
\item The source code and associated scripts are available at the Github repository. One can follow the instructions in the repo to verify the results in the paper. One needs to use the same hardware and software version, but this artifact is functional under more settings.
\end{enumerate}
 %STOP_LATEX

\paragraph{Author-Created or Modified Artifacts:}
\begin{verbatim}
Persistent ID: doi.org/10.5281/zenodo.5144378, 
\end{verbatim}
\begin{verbatim}
Github: github.com/BoyuanFeng/ArbitraryPrecision.git
Artifact name: APNN-TC
\end{verbatim}



\section*{Baseline experimental setup, and modifications made for the paper}


\paragraph{Relevant hardware details:} Intel Xeon Sliver 4110 CPU, NVIDIA RTX3090 GPU
\paragraph{Operating systems and versions:} Ubuntu-16.04
\paragraph{Compilers and versions:} nvcc-11.0, gcc-7.5, CMAKE-3.14







\paragraph{URL to output from scripts that gathers execution environment information}
\begin{verbatim}
github.com/YukeWang96/sc21\_AD/blob/master/output.log
\end{verbatim}

% \subsection{SUMMARY OF THE EXPERIMENTS REPORTED}
% The artifact contains the CUDA code for \Mname~described in our paper. In addition it contains
% the codes, shell scripts and instructions needed to carry out other
% experiments in the evaluation section of the paper, including
% \begin{enumerate}
%     \item We ran \Mname~on datasets from MNIST~(\textit{\url{https://en.wikipedia.org/wiki/MNIST_database}}), CIFAR~(\textit{\url{https://www.cs.toronto.edu/~kriz/cifar.html/}}), and ImageNet~(\textit{\url{http://www.image-net.org/}}) on NVIDIA RTX3090 GPU and Tesla A100 GPU, and record execution time of average of 200 runs, and compare with the baselines CUTLASS~\cite{cutlass} described in the paper. 
%     The program is compiled with CUDA-11.1. 
%     \item Baselines: we run GEMM and CONV example codes provided by CUTLASS-2.5.0 on RTX3090 and Tesla A100.
%     \item The source code and associated scripts are available at Github repo~(\textit{\url{}})\todo{add the url here}. 
%     One can follow the instructions in the repo to verify the results in the paper. One needs to use same hardware and software version, but this artifact is functional under more settings.
% \end{enumerate}


% \subsection{ARTIFACT AVAILABILITY}
% \hspace{6pt} \textbf{Software Artifact Availability:} 
% All author-created software artifacts are maintained in a public repository under an OSI-approved license.

% \textbf{Hardware Artifact Availability:} There are no author-created hardware artifacts.

% \textbf{Data Artifact Availability:} All author-created data artifacts are
% maintained in a public repository under an OSI-approved license.
% Proprietary Artifacts: No author-created artifacts are proprietary.

% \textbf{Author-Created or Modified Artifacts:} 
% Persistent ID: \todo{add the url here};
% Artifact name: APNN-TC code.

% \subsection{BASELINE EXPERIMENTAL SETUP, AND
% MODIFICATIONS MADE FOR THE PAPER}

% \hspace{6pt} \textbf{Relevant hardware details:} Intel Xeon Sliver 4110 CPU (8-core 16-threads) with 64GB host memory, NVIDIA RTX3090 GPU with 24 GB and Tesla A100 with 40GB device memory.

% \textbf{Operating systems and versions:} Ubuntu 16.04.

% \textbf{Compilers and versions:} NVCC-11.1, GCC-7.5.0

% \textbf{Libraries and versions:} CUDA-11.1, CUTLASS-2.5.0

% \textbf{Input datasets and versions:} MNIST, CIFAR, and ImageNet.

